Learning Gaussian Operations and the Matchgate Hierarchy

Learning an unknown quantum process is a central task for validation of the functioning of near-term devices. The task is generally hard, requiring exponentially many measurements if no prior assumptions are made on the process. However, an interesting feature of the classically-simulable Clifford group is that unknown Clifford operations may be efficiently determined from a black-box implementation. We extend this result to the important class of fermionic Gaussian operations. These operations have received much attention due to their close links to fermionic linear optics. We then introduce an infinite family of unitary gates, called the Matchgate Hierarchy, with a similar structure to the Clifford Hierarchy. We show that the Clifford Hierarchy is contained within the Matchgate Hierarchy and how operations at any level of the hierarchy can be efficiently learned.

==> input_files/background.tex <==
We first note that the Majorana monomials $\gamma_S = \gamma_{\mu_1}\ldots \gamma_{\mu_\abs{S}}$ for $S \subseteq [2n]$ form a basis of $\text{Mat}(2^n)$.
Therefore, knowing the action of $U \gamma_\mu U^\dag$ for each $\mu$ implies knowledge of the action of $U M U^\dag$ for any $M \in \text{Mat}(2^n)$.
This action uniquely determines $U$ up to an overall phase.

For Gaussian operations, we have $M \gamma_\mu M^\dag = \sum_{\nu} Q_{\mu \nu} \gamma_\nu$ for some matrix $Q \in O(2n)$.
So we seek to learn $Q$ in order to uniquely determine $M$.

Recall that a Gaussian operator is given by $M = e^{iH}$, where $H = i \sum_{\mu,\nu} h_{\mu \nu} \gamma_\mu \gamma_\nu$ is a quadratic Hamiltonian.
$h$ is such that $Q = e^{4h}$.

Recall also that for a (pure or mixed) Gaussian state $\rho$, the \emph{correlation matrix} $\Gamma(\rho)$ is defined by
$$
\Gamma(\rho)_{jk} \coloneqq
\langle i \gamma_j \gamma_k \rangle_\rho 
= \Tr\left(i \gamma_j \gamma_k \rho \right)
$$
Gaussian states are in 1-1 correspondence with valid correlation matrices -- real, anti-symmetric matrices with eigenvalues of modulus at most unity.

Further, the set of (mixed) Gaussian states are the closure of Gibbs states of quadratic Hamiltonians:
$$\rho_G = \frac{e^{-H}}{Tr(e^{-H})}.$$
We have that $\Gamma(\rho_G) = \tan(2h)$.

Throughout, let $M_Q$ be the operation which conjugates the $\gamma$s according to $Q$.
$M_Q$ is Gaussian iff $Q$ is orthogonal.

==> input_files/indirect.tex <==
We consider a 3-step learning process.
\begin{enumerate}
    \item We perform a direct sampling process of each row of $Q$ in turn, obtaining a guess $\tilde{Q}$, which is identical to $Q$ up to additive error $\epsilon$ and entry-wise incorrect signs.
    \item We use the framework of matchgate shadows to estimate $\Tr\left( M_{\tilde{Q}} \gamma_1 \gamma_2 M_{\tilde{Q}}^\dag \cdot M_Q \ket{0}\bra{0} M_Q^\dag \right)$ for each of the $2^{4n^2}$ possible choices of $\tilde{Q}$.
    This requires only polynomially many -- $\mathcal{O}(n^3)$ -- samples (though, of course, exponential time).
    The idea is that the true choice of $\tilde{Q} = Q$ leads to an expectation value of $i$, whereas incorrect choices will generally give different values.\\
    This will lead to a set of $2^n$ choices of $\tilde{Q}$, corresponding to the true $Q$ up to whole row sign changes.
    \item For one of the above guesses $\tilde{Q}$, prepare 
    $(M_{\tilde{Q}}^\dag \otimes I)\ket{\psi}$ and measure w.r.t. the basis 
    $\{ (\gamma_S M^\dag \otimes I)\ket{\psi} \}$, where $\ket{\psi} = 2^{-n/2}\sum_i \ket{ii}$ is the maximally entangled state. 
    The outcome of this measurement allows the guess to be corrected to the true $Q$.
\end{enumerate}

Problems:
\begin{itemize}
    \item Collection of errors -- how does imperfect knowledge of $Q$ (up to signs) impact the shadows?
    \item Can we guarantee that only the true $Q$ and its row-wise sign equivalent matrices $\tilde{Q}$ survive step 2? Some processing to remove diagonal parts of $Q$, or removing equivalent $\tilde{Q}$, should be done here.
    \item Although sample complexity is good, exponential time complexity is not ideal.
\end{itemize}
